UniVSE: Robust Visual Semantic Embeddings via Structured Semantic Representations

We propose Unified Visual-Semantic Embeddings (UniVSE) for learning a joint space of visual and textual concepts. The space unifies the concepts at different levels, including objects, attributes, relations, and full scenes. A contrastive learning approach is proposed for the fine-grained alignment from only image-caption pairs. Moreover, we present an effective approach for enforcing the coverage of semantic components that appear in the sentence. We demonstrate the robustness of Unified VSE in defending text-domain adversarial attacks on cross-modal retrieval tasks. Such robustness also empowers the use of visual cues to resolve word dependencies in novel sentences.

==> fig_text/adversarial_demo.tex <==
\begin{figure*}
	\vspace{-0.2in}
	\centering
	\includegraphics[width=170mm]{fig/adversarial_exp.pdf}
	\caption{Examples showing the top-5 image-to-text retrieval results with the presence of adversarial samples.
% 	The left one is under object attack and the right one is under relation attack.
    We highlight the positive captions in blue.
    Words in red indicates the irrelevant words in the adversarial captions. The score in the front of each sentence is the similarity score of the caption and image computed by different model.
    }
	\label{fig:adversarial_exp}
	\vspace{-0.1in} 
\end{figure*}

==> fig_text/global_retrieval.tex <==

\begin{table*}
	\vspace{-0.25in}
	\small
	\begin{center}
		\begin{tabular}{c|cccc||cccc||c}
			\hline
			Task & \multicolumn{4}{c||}{Image-to-sentence Retrieval} & \multicolumn{4}{c||}{Sentence-to-image Retrieval} &\\
			\hline
			Metric & R@1 & R@5 & R@10 & Med. r & R@1 & R@5 & R@10 & Med. r & rsum \\
			\hline
			\multicolumn{10}{c}{\textbf{1K testing split (5,000 captions)}}\\
			\hline
			m-RNN \cite{mrnn} & 41.0 & 73.0 & 83.5 & 2 & 29.0 & 42.2 & 77.0 & 3 & 345.7\\
			DVSA \cite{dvsa} & 38.4 & 69.9 & 80.5 & 1 & 27.4 & 60.2 & 74.8 & 3 & 351.2\\
			MNLM \cite{mnlm} & 43.4 & 75.7 & 85.8 & - & 31.0 & 66.7 & 79.9 &  - & 382.5\\
			m-CNN \cite{mcnn} & 42.8 & 73.1 & 84.1 & 3 & 32.6 & 68.6 & 82.8 & 3 & 384.0\\
			HM-LSTM\cite{hmlstm} & 43.9 & - & 87.8 & 2 & 36.1 & - & 86.7 & 3 & - \\
			Order-embedding \cite{oem} & 46.7 & - & 88.9 & 2 & 37.9 & - & 85.9 & 2 & - \\
% 			VSE-C(paper reported)\cite{vsec} & 50.2 & - & 89.8 & - & - & - & - & - & - \\
			VSE-C(open-source)\cite{vsec}\cite{vsec_github} & 48.0 & 81.0 & 89.2 & 2 & 39.7 & 72.9 & 83.2 & 2 & 414\\
			DeepSP\cite{deepsp} & 50.1 & 79.7 & 89.2 & - & 39.6 & 75.2 & 86.9 & - & 420.7\\
			2WayNet \cite{2waynet} & 55.8 & 75.2 & - & - & 39.7 & 63.3 & - & - & -\\	
			sm-LSTM \cite{smlstm} & 53.2 & 83.1 & 91.5 & 1 & 40.7 & 75.8 & 87.4 & 2 & 431.8\\
			RRF-Net\cite{rrfnet} & 56.4 & 85.3 & 91.5 & - & 43.9 & 78.1 & 88.6 & - & 443.8\\
% 			VSE++(paper reported, RC+rV)\cite{vsepp} & 58.3 & - & 93.3 & 1 & 43.6 & - & 87.8 & 2 & -\\
			VSE++(open-source)\cite{vsepp}\cite{vsepp_github} & 57.7 & 86.0 & 94.0 & 1 & 42.8 & 77.2 & 87.4 & 2 & 445.1 \\
			CSE\cite{cse} & 56.3 & 84.4 & 92.2 & 1 & 45.7 & 81.2 & 90.6 & 2 & 450.4\\
			%\modelshort(Ours) & \textbf{64.1} & \textbf{89.7} & \textbf{95.5} & \textbf{1} & \textbf{48.0} & \textbf{81.9} & \textbf{91.1} & \textbf{2} & \textbf{470.4} \\
			\modelshort(Ours) & \textbf{62.2} & \textbf{88.4} & \textbf{94.6} & \textbf{1} & \textbf{47.9} & \textbf{82.3} & \textbf{91.3} & \textbf{2} & \textbf{466.7} \\
			%\hline
			%Bean (RC+rV) & 69.8 & 91.9 & 96.6 & 1 & 55.9 & 86.9 & 94.0 & 1 & 495.1\\
			%Order & 69.9 & 92.9 & 97.5 & 1 & 56.7 & 87.5 & 94.8 & 1 & 499.3 \\
			\hline
			\multicolumn{10}{c}{\textbf{5K testing split (25,000 captions)}}\\
			\hline
			Order-embedding \cite{oem} & 23.3 & - & 65.0 & 5 & 18.0 & - & 57.6 & 7 & - \\
			VSE-C(open-source) \cite{vsepp}\cite{vsec_github} & 22.3 & 51.1 & 65.1 & 5 & 18.7 & 43.8 & 56.7 & 7 & 257.7\\
			CSE\cite{cse} & 27.9 & 57.1 & 70.4 & 4 & 22.2 & 50.2 & 64.4 & 5 & 292.2 \\
			VSE++(open-source) \cite{vsepp}\cite{vsepp_github} & 31.7 & 60.9 & 72.7 & 3 & 22.1 & 49.0 & 62.7 & 6 & 299.1 \\
			\modelshort(Ours) & \textbf{36.4} & \textbf{66.4} & \textbf{78.3} & \textbf{3} & \textbf{25.6} & \textbf{53.4} & \textbf{66.6} & \textbf{5} & \textbf{326.6} \\
			\hline
		\end{tabular}
	\end{center}
	%\vspace{-0.15in}	    
	\caption{\label{tab:overall_eval}Results of cross-modal retrieval task on MS-COCO dataset (1K and 5K testing split). All listed baselines and our models fix weights of the image encoders. For fair comparison, we do not include \cite{beans} and \cite{order} that finetunes the image encoder or adds extra training data.}
	\vspace{-0.15in}
\end{table*}


==> fig_text/model.tex <==
\begin{figure*}[t!]
	\centering
	\vspace{-0.2in}
	\includegraphics[width=170mm]{fig/model.pdf}
	\caption{{\bf Left}: the architecture of \model. 
	The semantic component alignment is learned from contrastive examples sampled from factorized semantic space. 
	The model also learns a caption encoder that combines the semantic components and aligns the caption with the corresponding image. 
	{\bf Right}: An exemplar computation graph for retrieving images from texts. The presence of $\txtglobal_{comp}$ in the caption encoding enforces the coverage of all semantic components. 
	See Sec. \ref{sec:local_learning} for details.}
	\label{fig:model}
	\vspace{-0.1in}
\end{figure*}

